Comparison of spectrogram scaling in multi-label Music Genre Recognition

As the accessibility and ease-of-use of digital audio workstations increases, so does the quantity of music available to the average listener; additionally, differences between genres are not always well defined and can be abstract, with widely varying combinations of genres across individual records. In this article, multiple preprocessing methods and approaches to model training are described and compared, accounting for the eclectic nature of today's albums. A custom, manually labeled dataset of more than 18000 entries has been used to perform the experiments.

==> abstract.tex <==
\abstract{
% English abstract 
In the current day and age, music is surrounding us everywhere, and accurate genre classification is important to both the recipients, as well as music labels and stores. However, due to many factors, nowadays the genres of songs and albums are not clearly defined, oftentimes mixed on a single record. That's why in this work an extensive comparison of various preprocessing methods and ways of handling imbalanced data is performed for a multi-label classification. For the experiments were used spectrograms extracted from audio files, where the dataset was personally acquired and labeled based on the biggest online music database, resulting in more than 18000 data.  

}{
% Abstract translated into Polish

W obecnych czasach, muzyka otacza nas ze wszystkich stron, a dokładna klasyfikacja gatunków muzycznych jest istotna dla zarówno odbiorcy, jak i wytwórni muzycznych czy sklepów. Jednak z wielu powodów obecnie gatunki piosenek czy całych albumów nie są ściśle zdefiniowane, a często jest to miks wielu na jednym utworze. Z tego powodu w tej pracy zostało przeprowadzone obszerne porównanie różnych metod wstępnej obróbki danych, jak i radzenia sobie z niezbalansowaniem danych dla wieloetykietowej klasyfikacji. Spektrogramy wyekstraktowane z plików muzycznych zostały użyte do eksperymentów, gdzie zbiór danych został zebrany osobiście, a etykiety zostały nadane bazując na największej internetowej muzycznej bazie danych, w rezultacie dając ponad 18000 danych.
}

==> analysis.tex <==
In order to assess the impact of using mel-scale and non-mel-scale spectrograms during the experiments, the F1 metric has been used as a point of comparison between the two. Aggregated performance values from transfer models have been considered in order to evaluate whether the choice of spectrogram type yields statistically different results.

For each type of spectrogram, aggregated F1 scores were obtained across the models. Because the aggregated values represent paired observations (that is, each model provides an F1 score for both spectrogram types), the difference in F1 scores (spectrogram F1 minus mel spectrogram F1) has been calculated for each model.

Before performing the main hypothesis test, the normality of these differences was assessed using the Shapiro–Wilk test, which failed to reject the null hypothesis of normality - as such, the differences appear approximately normally distributed. The Q-Q plot in Figure \ref{fig:qq} shows the differences against the theoretical quantiles of a "perfectly" normal distribution, showing only modest variations towards the extremes (which indicates normality). This confirmation of normality, combined with the paired nature of the compared data, narrowed the selection of the test to a paired t-test.

\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{results/qq-normal.pdf}
    \caption{Q–Q Plot for Differences in F1 between mel spectrograms and normal spectrograms}
    \label{fig:qq}
\end{figure}

% Po aktualizacji wyników - mamy dla porównania malutkie p
The results of the dependent samples t test ($p=0.0027$) indicate that there is a statistically significant difference between the two types of spectrograms, as far as their F1 scores are concerned in this highly varied dataset. The resulting t-statistic of $-3.5872$ is indicative of mel spectrograms that have an edge over normal scale spectrograms (in terms of F1 scores), which matches the a priori expectations of the experiment results.
